An $r$-adaptive finite element method using neural networks for parametric self-adjoint elliptic problem

This work proposes an $r$-adaptive finite element method (FEM) using neural networks (NNs). The method employs the Ritz energy functional as the loss function, currently limiting its applicability to symmetric and coercive problems, such as those arising from self-adjoint elliptic problems. The objective of the NN optimization is to determine the mesh node locations. For simplicity in two-dimensional problems, these locations are assumed to form a tensor product structure. The method is designed to solve parametric partial differential equations (PDEs). For each PDE parameter instance, the optimal $r$-adapted mesh generated by the NN is then solved with a standard FEM. The construction of FEM matrices and load vectors is implemented such that their derivatives with respect to mesh node locations, required for NN training, can be efficiently computed using automatic differentiation. However, the linear equation solver does not need to be differentiable, enabling the use of efficient, readily available `out-of-the-box' solvers. Consequently, the proposed approach retains the robustness and reliability guarantees of the FEM for each parameter instance, while the NN optimization adaptively adjusts the mesh node locations. The method's performance is demonstrated on parametric Poisson problems using one- and two-dimensional tensor product meshes.

==> figures/example_III_1a/figure_solutions3d_32.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/example_III_1a/sigma1.png}
    \caption{Caption}
    \label{fig:exIII1a_solution}
\end{figure}

==> tables/example_I_2b/table_stats_lin.tex <==

\begin{table}[h]
    \centering
    \caption{Example I 2 b, error metrics training in linspace }
    \label{tab:errors_lin}
    % \vspace{0.5cm}
    \pgfplotstabletypeset[
        col sep=comma,
        header=true,
        every head row/.style={before row=\toprule, after row=\midrule},
        every last row/.style={after row=\bottomrule},
        columns/Set/.style={string type},
        columns/Mean Absolute Error/.style={
            column name=\makecell{Mean \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Mean Relative Error (per)/.style={
            column name=\makecell{Mean Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Std Absolute Error/.style={
            column name=\makecell{Std \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Std Relative Error (per)/.style={
            column name=\makecell{Std Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Max Absolute Error/.style={
            column name=\makecell{Max \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Max Relative Error (per)/.style={
            column name=\makecell{Max Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        }
    ]{data/example_I_2b/Error_result_lin.csv}
\end{table}

==> tables/example_I_2b/table_stats_log.tex <==

\begin{table}[h]
    \centering
    \caption{Example I 2 b, error metrics training in logspace }
    \label{tab:errors_log}
    % \vspace{0.5cm}
    \pgfplotstabletypeset[
        col sep=comma,
        header=true,
        every head row/.style={before row=\toprule, after row=\midrule},
        every last row/.style={after row=\bottomrule},
        columns/Set/.style={string type},
        columns/Mean Absolute Error/.style={
            column name=\makecell{Mean \\ Abs. Error},
            sci, sci sep align, precision=3
        },
        columns/Mean Relative Error (per)/.style={
            column name=\makecell{Mean Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Std Absolute Error/.style={
            column name=\makecell{Std \\ Abs. Error},
           sci, sci sep align, precision=3
        },
        columns/Std Relative Error (per)/.style={
            column name=\makecell{Std Rel. \\ Error (\%)},
           % sci, sci sep align, 
           precision=3
        },
        columns/Max Absolute Error/.style={
            column name=\makecell{Max \\ Abs. Error},
            sci, sci sep align, precision=3
        },
        columns/Max Relative Error (per)/.style={
            column name=\makecell{Max Rel. \\ Error (\%)},
           % sci, sci sep align, 
           precision=3
        }
    ]{data/example_I_2b/Error_result_log.csv}
\end{table}


==> tables/example_I_3b/table_stats_lin.tex <==

\begin{table}[h]
    \centering
    \caption{Example I 3 b, error metrics training in linspace }
    \label{tab:errors_lin}
    % \vspace{0.5cm}
    \pgfplotstabletypeset[
        col sep=comma,
        header=true,
        every head row/.style={before row=\toprule, after row=\midrule},
        every last row/.style={after row=\bottomrule},
        columns/Set/.style={string type},
        columns/Mean Absolute Error/.style={
            column name=\makecell{Mean \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Mean Relative Error (per)/.style={
            column name=\makecell{Mean Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Std Absolute Error/.style={
            column name=\makecell{Std \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Std Relative Error (per)/.style={
            column name=\makecell{Std Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Max Absolute Error/.style={
            column name=\makecell{Max \\ Abs. Error},
            sci, sci sep align, 
            precision=3
        },
        columns/Max Relative Error (per)/.style={
            column name=\makecell{Max Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        }
    ]{data/example_I_3b/Error_result_13_lin.csv}
\end{table}

==> tables/example_I_3b/table_stats_log.tex <==

\begin{table}[h]
    \centering
    \caption{Example I 3 b, error metrics training in logspace }
    \label{tab:errors_log}
    % \vspace{0.5cm}
    \pgfplotstabletypeset[
        col sep=comma,
        header=true,
        every head row/.style={before row=\toprule, after row=\midrule},
        every last row/.style={after row=\bottomrule},
        columns/Set/.style={string type},
        columns/Mean Absolute Error/.style={
            column name=\makecell{Mean \\ Abs. Error},
            sci, sci sep align, precision=3
        },
        columns/Mean Relative Error (per)/.style={
            column name=\makecell{Mean Rel. \\ Error (\%)},
            % sci, sci sep align, 
            precision=3
        },
        columns/Std Absolute Error/.style={
            column name=\makecell{Std \\ Abs. Error},
           sci, sci sep align, precision=3
        },
        columns/Std Relative Error (per)/.style={
            column name=\makecell{Std Rel. \\ Error (\%)},
           % sci, sci sep align, 
           precision=3
        },
        columns/Max Absolute Error/.style={
            column name=\makecell{Max \\ Abs. Error},
            sci, sci sep align, precision=3
        },
        columns/Max Relative Error (per)/.style={
            column name=\makecell{Max Rel. \\ Error (\%)},
           % sci, sci sep align, 
           precision=3
        }
    ]{data/example_I_3b/Error_result_13_log.csv}
\end{table}


% {data/example_I_3b/Error_result.csv}
